Quantum software experiments: A reporting and laboratory package structure guidelines

Background. In the realm of software engineering, there are widely accepted guidelines for reporting and creating laboratory packages. Unfortunately, the landscape differs considerably in the emerging field of quantum computing. To the best of our knowledge, no standardized guidelines exist for describing experiments or outlining the necessary structures for quantum software laboratory packages. Aims. This paper endeavors to enhance the replicability and verifiability of quantum software experiments. Method. This objective is pursued through the proposition of guidelines for reporting and the delineation of a structure for laboratory packages tailored to quantum computing experiments. Specifically, we advocate for an extension and adaption of established guidelines in experimental software engineering, integrating novel elements to address the specific requirements of quantum software engineering. Results. In validating the utility and effectiveness of the proposed guidelines, we conducted a review encompassing 11 works (5 focusing on reporting guidelines and 6 on laboratory packages). In particular, this review highlighted the absence of standardized guidelines and structure of laboratory packages for quantum software experiments. Conclusions. Our assessment revealed gaps in information and opportunities for enhancement within the evaluated papers and laboratory packages. Our proposal contributes to the advancement of quantum software engineering research, taking a fundamental step toward fostering rigorous and reliable scientific research in this emerging paradigm.

==> old-intro.tex <==
\section{Introduction}
\label{sec:introduction}

% Submissions to this track are limited to 10 pages excluding references and 12 pages with references and must be submitted through EasyChair by selecting the track “Technical Papers.”

The Open Science movement actively advocates greater transparency in scientific research, promoting the replicability of studies as a means of validating findings and reinforcing theoretical foundations \cite{Barba2019}. Facilitating the accessibility of research and its accompanying supplementary materials to the scientific community encourages opportunities for reanalysis, enhancing the dependability of results. Furthermore, this approach empowers emerging researchers to replicate studies by providing unrestricted access to the utilized materials, enabling subsequent consultation and reuse. In essence, Open Science endeavors to augment the transparency, reproducibility, and replicability of empirical research \cite{Shull2008}.

%More specifically, Empirical Software Engineering constitutes a specialized field of research that advocates for the application of the experimental scientific method to derive insights into the software development process. Although the use of the experimental method is a customary practice in various scientific domains, its integration into software engineering research is a relatively recent development. The inception of this field traces back to the 1970s, marked by several propositions endorsing the empirical observation of software development methodologies \cite{Hey2015computing}. Nevertheless, the formalization and initiation of experiments applying the scientific method in the realm of software engineering are attributed to Basili, with pioneering work commencing in 1984 \cite{Basili1984methodology}.

An experiment involves the deliberate manipulation and observation of real-world conditions to conduct an in-depth examination of a particular phenomenon. It serves as a systematic endeavor to discern relationships among the variables pertinent to the studied phenomenon.  In the domain of software development, experimentation, although still evolving, has commenced as a method to substantiate or challenge assertions about techniques and tools employed in the construction of software \cite{juristo2013basics}. 
Consequently, appropriate reporting of the details of the experiment, its context, execution, and results, is essential for ensuring its validity and replicability.  The establishment of comprehensive reporting guidelines plays as a consequence a pivotal role in empirical research, serving as a cornerstone for enhancing the transparency, reproducibility, and validity of findings. These guidelines are instrumental in ensuring that researchers provide a complete, clear, and systematic account of their experimental designs, conduction details, data analyses, and findings. 

In the area of Empirical Software Engineering, reporting guidelines for different kinds of studies were proposed decades ago \cite{jedlitschka2008reporting,kitchenham2008evaluating,kitchenham2007guidelines} and are actively maintained and improved \cite{kitchenham2023guidelines}. Despite the benefits of following such guidelines, their actual adoption and the consistency of reporting practices in software engineering experiments have usually been questioned. Research indicates that many experimental papers in software engineering fail to adhere to these guidelines, with a significant number of papers not citing any guidelines at all \cite{Revoredo2021}. 
In this context, a Laboratory Package (LP) is a collection of artifacts systematically employed throughout the entire lifecycle of an experiment, encompassing the stages of planning, execution, and analysis \cite{Shull2002}.
The Empirical Software Engineering community has proactively put forth multiple propositions about the standardization and generation of LPs \cite{Guevara2021,Solari2018}. These proposals aim to establish uniformity and provide guidelines for the systematic creation of comprehensive sets of artifacts essential for conducting empirical studies in the software engineering domain.

% Nevertheless, a novel computing paradigm is on the horizon, poised to reshape the landscape of Software Engineering in the foreseeable future: Quantum Computing. 
Quantum computing is an emergent paradigm that holds the potential to address challenges that conventional computing, in its current form, struggles to resolve within a practical timeframe \cite{Harrow2017}. Quantum Computing introduces a paradigm shift by harnessing the principles of quantum mechanics, offering the prospect of tackling computational problems that were previously deemed insurmountable within traditional computing frameworks.

Today, there are already advances in the field of Quantum Software Engineering and there are technological proposals and experiments in this new field of Software Engineering \cite{Serrano2022}. But as with traditional Empirical Software Engineering, the conduction of an experiment in Quantum Software Engineering has conceptual and material barriers that must be addressed %\cite{Moguel2020}
\cite{Piattini2020}. To perform such experiments, researchers must handle a number of concepts intrinsic to quantum computing. From a material point of view, such an experiment will require a quantum computer, which usually involves using such hardware owned by other organizations as a service on a pay-per-use basis (or using simulations). For these reasons, experimentation in the field of quantum computing is different with respect to experimentation in classical software engineering and therefore requires new techniques/mechanisms/methodologies and/or adapting existing ones to the new characteristics of this new computing paradigm.

A \emph{Quantum Software Experiment (QSE)} is characterized by the involvement of quantum software in the experimental framework, which can play a variable role. This role may range from a critical element, pivotal to the experiment's objectives and variables, to a more nuanced function. %In scenarios where quantum software is central, the experiments typically focus on evaluating and comparing the effects of quantum and classical algorithms or implementations.

For QSEs, the reporting and replicability problem is even more challenging. The current state of quantum computing entails that software is often developed through the specification of circuits based on logic gates, and not all quantum software can be executed on any of the existing quantum computers due to the significant technological diversity \cite{alvarado2023}. These hurdles have led to various proposals being put forward to facilitate the task of executing and deploying quantum software %\cite{Romero-Alvarez2023,alvarado2023,romero2023}
\cite{Romero-Alvarez2023,alvarado2023}, but they also affect the requirements for reporting QSEs, threatening their replicability. %One of the ways to enhance reporting and replicability of empirical studies is through the use of reporting guidelines.

In this work, we aim to facilitate the replication of QSEs.
Despite the unique characteristics and complexities associated with quantum software that demands meticulous attention in experimental reporting, there remains a noticeable absence of tailored guidelines.  This paper tries to fill this gap, developing specific reporting guidelines based on the previous generic proposals created for empirical software engineering, and addressing the nuanced requirements of quantum computing research. 
To fully satisfy this objective, we not only propose a set of guidelines for the reporting of quantum software experiments, but we also outline a laboratory package structure for experiments in this area.

Therefore, this paper's contributions are twofold: Firstly, it offers an extension of the established reporting guidelines for software engineering experiments stated in \cite{jedlitschka2008reporting}, specifically tailored for quantum software engineering (Section \ref{Reporting}). This adaptation addresses the unique challenges and requirements of the quantum computing field. Secondly, it proposes a comprehensive LP structure, encompassing all necessary components for conducting and replicating experiments in quantum computing (Section \ref{LaboratoryPackage}). This package aims to facilitate rigorous and reproducible research within this emerging area.

% Until now, there are very few experiments that make use of quantum computation, and almost no public laboratory packages that can be used to replicate this type of experiment. That is why, I

The rest of the paper is structured as follows: Section \ref{sec:background} provides an overview of essential quantum computing concepts and relevant previous studies. Sections \ref{Reporting}  and \ref{LaboratoryPackage} present respectively our proposed experiment reporting guidelines and proposed integrated LP structure for the quantum software engineering domain. Section \ref{sec:validation} details the validation carried out for our proposal. Finally, Section \ref{sec:conclusion} presents a discourse on the implications and conclusions drawn from our research.

==> related-work-guidelines.tex <==
%\subsection{Guidelines for software engineering experiments reporting and LP structure}

